Trade-offs between classical and quantum space using spooky pebbling

Pebble games are used to study space/time trade-offs. Recently, spooky pebble games were introduced to study classical space / quantum space / time trade-offs for simulation of classical circuits on quantum computers. In this paper, the spooky pebble game framework is applied for the first time to general circuits. Using this framework we prove an upper bound for quantum space in the spooky pebble game. We also prove that solving the spooky pebble game is PSPACE-complete. Moreover, we present a solver for the spooky pebble game based on satisfiability solvers combined with heuristic optimizers. This spooky pebble game solver was empirically evaluated by calculating optimal classical space / quantum space / time trade-offs. Within limited runtime, the solver could find a strategy reducing quantum space when classical space is taken into account, showing that the spooky pebble model is useful to reduce quantum space.

==> DAG_example_uncomp.tex <==

\node[text=black] (txt) at (\hshift,1+\vshift) {(\lbl)};

\Colors{\1}
\node[shape=circle,draw=black,text=\TextColor,fill=\FillColor] (1) at (0+\hshift,0+\vshift) {A};

\Colors{\2}
\node[shape=circle,draw=black,text=\TextColor,fill=\FillColor] (2) at (\hdist+\hshift,0+\vshift) {B};

\Colors{\3}
\node[shape=circle,draw=black,text=\TextColor,fill=\FillColor] (3) at (0.5*\hdist+\hshift,1+\vshift) {C};


\path [->](1) edge (3);
\path [->](2) edge (3);



==> macros.tex <==
\usepackage{graphicx}
\usepackage{amsmath,dsfont}
\usepackage{amsthm}


\usepackage{comment}
\usepackage[noend]{algpseudocode}
\usepackage{algorithm}
\usepackage{hyperref}
\usepackage{marvosym}
\usepackage{placeins}
\usepackage{wrapfig}
\usepackage{cutwin}

\usepackage[numbers]{natbib}

\usepackage{booktabs}

\usepackage{tikz}
\usetikzlibrary{quantikz}
\usepackage{ifthen}

\RequirePackage{xspace}
\RequirePackage{amssymb}
\RequirePackage{amsfonts}

\newcommand\defaccr[2]{\newcommand#1{#2\xspace}}
\newcommand\defmath[2]{\newcommand#1{\ensuremath{#2}\xspace}}
\newcommand\concept[1]{\textit{#1}}


\defmath{\defn}{\,\triangleq\,}



\renewcommand\dots{\makebox[.7em][c]{.\hfil.\hfil.}}


\theoremstyle{plain}\newtheorem{note}[thm]{Note} 

\makeatletter
\patchcmd{\ALG@step}{\addtocounter{ALG@line}{1}}{\refstepcounter{ALG@line}}{}{}
\newcommand{\ALG@lineautorefname}{Line}
\makeatother
\newcommand{\alglineautorefname}{Line}

\newcommand\obj[1]{\textbf{Obj.~#1}}
\newcommand\task[1]{\textbf{Task~#1}}


\newcommand{\cbox}[2][yellow]{%
  \colorbox{#1}{\parbox{\dimexpr\linewidth-2\fboxsep}{\strut #2\strut}}%
}


\renewcommand\phi{\varphi}



\newcommand\ccode[1]{\texttt{#1}} 


\newcommand{\overarrowi}[1]{\xrightarrow{#1}}
\newcommand{\overarrow}[1]{
  \mathchoice{\raisebox{-3pt}{ $\overarrowi{#1}$ }}
             {\raisebox{-3pt}{ $\overarrowi{#1}$ }}
             {\raisebox{-3pt}{ $\overarrowi{#1}$ }}
             {\raisebox{-3pt}{ $\overarrowi{#1}$ }}}

\let\set\undefined

\providecommand{\tuple}[1]{\ensuremath{\left( #1 \right)}}
\providecommand{\set}[1]{\ensuremath{\left\lbrace #1 \right\rbrace}}
\providecommand{\sequence}[1]{\ensuremath{\left( #1 \right)}}
\providecommand{\sizeof}[1]{\ensuremath{\left\vert{#1}\right\vert}}
\providecommand{\vect}[1]{\ensuremath{( \begin{matrix} #1 \end{matrix} )}}
\providecommand{\always}[1]{\ensuremath{\left[ #1 \right]}}
\newcommand{\powerset}[1]{\ensuremath{\mathbf{2}^{#1}}}
\newcommand{\eval}[1]{\ensuremath{\llbracket #1\rrbracket}}
\newcommand{\qeval}[1]{\ensuremath{\ket{#1}}}


\providecommand{\gen}[1]{\ensuremath{\left\langle #1 \right\rangle}}



\newcommand{\id}[1][]{\ensuremath{\mathbb{I}_{#1}}\xspace}
\defmath{\bool}{\ensuremath{\mathbb{B}}}
\defmath{\nat}{\ensuremath{\mathbb{N}}}
\defmath{\complex}{\ensuremath{\mathbb{C}}}
\defmath{\real}{\ensuremath{\mathbb{R}}}
\defmath{\integers}{\ensuremath{\mathbb{Z}}}


\newcommand{\bracket}[1]{\left(#1\right)}
\newcommand{\underbraceset}[2]{\underset{#1}{\underbrace{#2}}}
\newcommand{\rfrac}[2]{\ ^{#1} \!/_{#2}}
\newcommand{\atmost}[1]{\ensuremath{\mathcal{O}(#1)}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}


\defmath\Exists{\mathit{Exists}}
\defmath\PlusExists{\mathit{PlusExists}}
\defmath\var{\mathit{var}}
\defmath\calciso{\mathsf{calciso}}



\providecommand{\abs}[1]{\lvert#1\rvert}


\newcommand{\turner}[3][10em]{%
  \rlap{\rotatebox{#2}{\begin{varwidth}[t]{#1}#3\end{varwidth}}}%
}

\newcommand\local[5]{\begin{smallmat}#5{#1} & #5{#2} \\ #5{#3} & #5{#4}\end{smallmat}\xspace}
\newcommand\anti[1]{\begin{smallmat}0 & #1 \\ 1 & 0\end{smallmat}\xspace}
\newcommand\diag[1]{\begin{smallmat}1 & 0 \\  0 & #1\end{smallmat}\xspace}

\newcommand\diagg[2]{\begin{smallmat}#1 & 0 \\  0 & #2\end{smallmat}\xspace}



\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


\defmath\yy{\begin{smallmat}
    0 & y^*\\
    y & 0\\
\end{smallmat}}

\defmath\ww{\begin{smallmat}
      0 & y   \\
      y^* & 0  \\
  \end{smallmat}
}


\newcommand{\TextColor}{black}
\newcommand{\FillColor}{white}

\newcommand{\Colors}[1]{\ifthenelse{#1 = 0}{
        \renewcommand{\TextColor}{black}
        \renewcommand{\FillColor}{white}
    }{}
    \ifthenelse{#1 = 1}{
        \renewcommand{\TextColor}{white}
        \renewcommand{\FillColor}{black}
    }{}
    \ifthenelse{#1 = 2}{
        \renewcommand{\TextColor}{black}
        \renewcommand{\FillColor}{gray}
    }{}
}

\newcommand{\PSPACE}{\textsf{PSPACE}}
\newcommand{\NPSPACE}{\textsf{NPSPACE}}

%\renewcommand\UrlFont{\color{blue}\rmfamily}      % By LMCS standard url color is black. If you do not agree with this, let us know.


